Cross-Modality Program Representation Learning for Electronic Design Automation with High-Level Synthesis

In recent years, domain-specific accelerators (DSAs) have gained popularity for applications such as deep learning and autonomous driving. To facilitate DSA designs, programmers use high-level synthesis (HLS) to compile a high-level description written in C/C++ into a design with low-level hardware description languages that eventually synthesize DSAs on circuits. However, creating a high-quality HLS design still demands significant domain knowledge, particularly in microarchitecture decisions expressed as \textit{pragmas}. Thus, it is desirable to automate such decisions with the help of machine learning for predicting the quality of HLS designs, requiring a deeper understanding of the program that consists of original code and pragmas. Naturally, these programs can be considered as sequence data. In addition, these programs can be compiled and converted into a control data flow graph (CDFG). But existing works either fail to leverage both modalities or combine the two in shallow or coarse ways. We propose ProgSG, a model that allows interaction between the source code sequence modality and the graph modality in a deep and fine-grained way. To alleviate the scarcity of labeled designs, a pre-training method is proposed based on a suite of compiler's data flow analysis tasks. Experimental results show that ProgSG reduces the RMSE of design performance predictions by up to $22\%$, and identifies designs with an average of $1.10\times$ and $1.26\times$ (up to $8.17\times$ and $13.31\times$) performance improvement in design space exploration (DSE) task compared to HARP and AutoDSE, respectively.

==> sec-ablation.tex <==
\section{Ablation Study} %\YS{the introduction is too long. compress the DSA part.}
\label{sec-ablation}

\textbf{Effect of pre-training for the source code transformer} \enspace As shown in Table~\ref{table-abl-src-rand}, if we fine-tune a randomly initialized \src model (i.e. we load the pre-trained \src model\footnote{\url{https://huggingface.co/Salesforce/codet5-small}} but then randomly initialize all the encoder layers), the final result is much worse compared to starting the fine-tuning from a released checkpoint. Such an experiment confirms the usefulness of pre-training for the transformer encoder on our specific task. In addition, it suggests that to achieve low prediction error on our task, the encoder should be powerful enough, e.g. pre-trained on a large code corpus as done by \src. It further implies that the GNN model to encode the CDFG modality could also benefit from pre-training, which leads to the next ablation sudy

\begin{table*}[h]
\footnotesize
  \begin{center}
    \caption{Ablation study results on \vTwoTrue. Fine-tuning on a randomly initialized \src vs a pre-trained \src.
    }
    \begin{tabular}{l|ll}
    \label{table-abl-src-rand}
    \textbf{Method} &
    \textbf{Transductive} &
    \textbf{Inductive} \\
      \hline
    \srcRand  & 2.1363  & 2.5204 \\
    \src  &  0.4539 & 1.1837 \\
    \end{tabular}
  \end{center}
% \vspace*{-4mm}
\end{table*}


\textbf{Effect of pre-training for the GNN} \enspace As shown in Table~\ref{table-abl-pt}, if we do not start fine-tuning with any pre-trained GNN, i,e. we start with a randomly initialized GNN model, the result becomes worse. To further validate the usefulness of the proposed pre-training method, we compare our method with the state-of-the-art self-supervised GNN pre-training framework, \textsc{GraphMAE}~\cite{hou2022graphmae}. \textsc{GraphMAE} adopts a feature reconstruction task with both a node masking strategy and scaled cosine error loss to pre-train GNNs. The performance is shown in Table \ref{table-abl-pt}. We can see that the errors are close to the GNN without pre-training and are larger than our pre-training methods. It demonstrates that the pre-training framework designed for general purposes are not as effective as our method that is specifically designed for program graph.
%\yba{TODO: describe what is GraphMAE in details here}

\begin{table*}[h]
\footnotesize
  \begin{center}
    \caption{Ablation study results on \vTwoTrue. Comparing different pre-training schemes.
    }
    \begin{tabular}{l|ll}
    \label{table-abl-pt}
    \textbf{Method} &
    \textbf{Transductive} &
    \textbf{Inductive} \\
      \hline
    \modelNoPt  & 0.5043	& 1.3057 \\
  \modelgraphmae   & 0.5345 & 1.0306   \\
  \model & 0.3607 & 0.8199 \\

    \end{tabular}
  \end{center}
% \vspace*{-4mm}
\end{table*}



% \textbf{Effect of graph-summary-augmented sequence representation} \enspace As shown in Table~\ref{table-abl-si}, the techniques proposed in Section 3.2, 

% \begin{table*}[h]
% \footnotesize
%   \begin{center}
%     \caption{Ablation study results on \vTwoTrue. Removing graph-summary augmentation as input to the transformer leads to worse performance.
%     }
%     \begin{tabular}{l|ll}
%     \label{table-abl-si}
%     \textbf{Method} &
%     \textbf{Transductive} &
%     \textbf{Inductive} \\
%       \hline
%     \modelNoSI  & 0.5146	& 0.9772 \\
%   \modelTakeZero & 0.5625 & 0.9536 \\
%   \modelTakeOne & 0.4640 & 0.9451 \\
%    \sumInt & 0.4326 & 0.8743 \\

%     \end{tabular}
%   \end{center}
% % \vspace*{-4mm}
% \end{table*}



\textbf{Effect of the proposed node-token message passing mechanism} \enspace As shown in Table~\ref{table-abl-ntmp}, without using any alignment information (while keeping the rest of the model architecture identical to \model), the result becomes worse. Only using 50\% of the aligned node-token pairs leads to a better inductive result but an even worse transductive result compared with \modelNoNTMP. This may be attributed to the missing alignment information causing additional difficulty for the model to generalize to seen programs' designs, suggesting the necessity of using the original full amount of alignment information. As mentioned previously, we also experimented with augmentation techniques for the alignment, leading to worse results, again suggesting the necessity of utilizing the correct and full alignment information indicated by the assembly code obtained via setting the ``\texttt{--emit-llvm -g -S -c}'' compiler flags.

At this point, it is worth noting the difference between \modelNoNTMP and \sumInt. The former differs from \model only in the removal of node-token message passing, i.e. it still has $L_1=8$ GNN layers and $L_2=6$ additional GNN and transformer layers; In contrast, the latter not only lacks the node-token message passing, but also lacks the additional $L_2=6$ GNN layers, i.e. \sumInt first runs $L_1=8$ GNN layers, feeds the summary-augmented sequence into a $L_2=6$-layer transformer, and eventually presents the $\bm{h}_{\mathrm{cdfg}}$ and $\bm{h}_{\mathrm{src}}$ (which has absorbed information from $\bm{h}_{\mathrm{cdfg}}$ as shown in Equation (2) of the main paper) into the decoder. It turns out that \sumInt performs worse in the transductive setting but better in the inductive setting compared to \modelNoNTMP, showing that simply feeding the node embeddings of \sumInt into an additional $L_2=6$ GNN layers without any node-token message passing cannot improve the results. In other words, the node-token message passing is needed together with the additional $L_2=6$ GNN layers in order to obtain the best results under both settings.

\begin{table*}[h]
\footnotesize
  \begin{center}
    \caption{Ablation study results on \vTwoTrue. Removing node-token message passing leads to worse performance.
    }
    \begin{tabular}{l|ll}
    \label{table-abl-ntmp}
    \textbf{Method} &
    \textbf{Transductive} &
    \textbf{Inductive} \\
      \hline
    \sumInt & 0.4326 & 0.8743 \\
    \modelNoNTMP  & 0.3958	& 0.9940 \\
    \modelHoldOutFifty  & 0.464	& 0.9690 \\
    \model & 0.3607 & 0.8199 \\


    \end{tabular}
  \end{center}
% \vspace*{-4mm}
\end{table*}


\textbf{Effect of the number of GNN layers} \enspace As shown in Table~\ref{table-abl-gnnlayers}, more GNN layers lead to better results, due to the more powerful model. It is note worthy that all the methods in Table~\ref{table-abl-gnnlayers} use the guidance loss to take advantage of the pre-trained GNN model for fairness. In other words, our proposed pre-training techniques in Section 3.4 is architecture-agnostic -- As long as there is a GNN-based encoder for the CDFGs, one can use $\mathcal{L}_{\mathrm{guide}}$ to guide that GNN encoder. However, with more GNN layers, the encoder becomes more expressive, therefore achieving better results. In short, more GNN layers and pre-training are orthogonal to each other and both improve the overall performance.

\begin{table*}[h]
\footnotesize
  \begin{center}
    \caption{Ablation study results on \vTwoTrue. Fewer GNN layers, i.e. smaller $L_1$, leads to worse performance.
    }
    \begin{tabular}{l|ll}
    \label{table-abl-gnnlayers}
    \textbf{Method} &
    \textbf{Transductive} &
    \textbf{Inductive} \\
      \hline
  \model-$L_1=4$ & 0.8069 & 1.0035 \\
  \model-$L_1=6$ & 0.4854 & 0.8457 \\
   \model & 0.3607 & 0.8199 \\

    \end{tabular}
  \end{center}
% \vspace*{-4mm}
\end{table*}

\textbf{Effect of the sequence length} \enspace As shown in Table~\ref{table-abl-maxlen}, a shorter maximum sequence length, i.e. the maximum number of tokens in each subsequence as mentioned in Section~\ref{sec-details}, leads to worse results, which is expected due to the shorter attention span of the \src transformer encoder. However, this study also suggests the future possibility of designing efficient and effective techniques to handle long input code sequences, which could further bring benefit to the performance. Another implication is that, it could be advantageous to use a more expressive code transformer, which under the same maximum sequence length can improve the results with the cost of more resource usage to train such a transformer, transitioning into the next ablation study.

\begin{table*}[h]
\footnotesize
  \begin{center}
    \caption{Ablation study results on \vTwoTrue. Reducing the maximum sequence length for the source code from 64 to 32 leads to worse performance.
    }
    \begin{tabular}{l|ll}
    \label{table-abl-maxlen}
    \textbf{Method} &
    \textbf{Transductive} &
    \textbf{Inductive} \\
      \hline
  \model-$\mathrm{maxLen}=32$ & 0.4329 & 0.9960 \\
   \model & 0.3607 & 0.8199 \\

    \end{tabular}
  \end{center}
% \vspace*{-4mm}
\end{table*}


\textbf{Effect of the sequence length} \enspace As shown in Table~\ref{table-abl-tfmodel}, with a more expressive transformer model pre-trained on source code corpus, i.e. \graphcodebert~\cite{guo2020graphcodebert}, the results indeed become better. However, it is noteworthy that the goal of this paper is \textit{\textbf{not}} to obtain the lowest prediction error. We leave that as future efforts due to the tremendous of computational resources it potentially may consume. Instead, our paper shows the usefulness of using sequence-augmentation and node-token message passing together with pre-training GNNs under rigorous comparison, e.g. controlling the transformer model to be \src consistently except in this ablation study. In future, if a more powerful transformer is used, e.g. \src-\textsc{large}\footnote{\url{https://huggingface.co/Salesforce/codet5-large}}, we expect better performance in general for all of the methods compared in the main paper. At this point, it is also worth emphasizing the fact that all of the models fit into one single GPU for training and inference, and we report more details in Section~\ref{sec-cost}.


\begin{table*}[h]
\footnotesize
  \begin{center}
    \caption{Ablation study results on \vTwoTrue. Using a different source code encoder (\graphcodebert) with a larger embedding dimension ($d)$ and more self-attention layers  ($L_2$ leads to better performance with more memory usage and longer training and inference time.
    }
    \begin{tabular}{l|llllll}
    \label{table-abl-tfmodel}
    \textbf{Method} &
    \textbf{Transductive} &
    \textbf{Inductive} & \textbf{$d$} & \textbf{$L_2$} & \textbf{Parameter Size} & \textbf{Vocab Size}\\
      \hline

   \src &  0.4539 & 1.1837 & 512 & 6 & 168.733 MB & 32100 \\
   \graphcodebert & 0.3221 & 0.9192 & 768 & 12 & 550.722 MB & 50265 \\

    \end{tabular}
  \end{center}
% \vspace*{-4mm}
\end{table*}


\textbf{Effect of the GNN model architecture choice} \enspace As shown in Table~\ref{table-abl-gnnmodel}, \tfconv with \textsc{GAT} leads to worse results.


\begin{table*}[h]
\footnotesize
  \begin{center}
    \caption{Ablation study results on \vTwoTrue. Using \textsc{GAT} instead of \tfconv leads to worse performance.
    }
    \begin{tabular}{l|ll}
    \label{table-abl-gnnmodel}
    \textbf{Method} &
    \textbf{Transductive} &
    \textbf{Inductive} \\
      \hline

   \cdfgGAT &  2.1832 & 1.2692  \\
   \cdfg & 0.6547 &  1.1216 \\

    \end{tabular}
  \end{center}
% \vspace*{-4mm}
\end{table*}

==> sec-cost.tex <==
\section{Training Cost}
\label{sec-cost}


We report the training cost in Table~\ref{table-cost}, which also serves as a running time study to examine the efficiency of and overhead incurred by the proposed techniques. The parameter size is measured by looping through all learnable parameters of the model, and adding up the estimated sizes, where the estimation is performed by multiplying the number of elements (\texttt{numel} in PyTorch) by the size in bytes of an individual element (\texttt{element\_size} of PyTorch). The total estimated size is converted into megabytes (MB) for display. As mentioned in the main paper, each method is fine-tuned on our regression task for 1000 epochs, and thus the average time per epoch during training is reported.



\begin{table*}[h]
\footnotesize
  \begin{center}
    \caption{Training cost of different models on \vTwoTrue.
    }
    \begin{tabular}{l|ll}
    \label{table-cost}
    \textbf{Method} &
    \textbf{Parameter Size} &
    \textbf{Time per Training Epoch}  \\
    % & 50 & 100 & 50 & 100 & 50 & 100 \\
      \hline
    \codeTwoVec & 2.363 MB	& 5.963 sec \\
    \src     &  168.733 MB & 1.000 min, 43.931 sec   \\
    \cdfg     & 35.533 MB & 1.000 min, 52.457 sec   \\
    \hline     
    \greaseLM & 322.545 MB	& 3.000 mins, 16.034 sec \\
    \simpleConcat  & 231.692 MB &	2.000 mins, 3.960 secs     \\
    \sumInt & 233.569 MB	 & 6.000 mins, 34.623 sec \\
    \model & 327.174 MB & 7.000 mins, 14.218 secs
    \end{tabular}
  \end{center}
% \vspace*{-4mm}
\end{table*}


It is noteworthy that \codeTwoVec is the fastest method. This is because we only report the fine-tuning process which receives one embedding per design generated by the released \codeTwoVec model, and the entire fine-tuning process only applies the MLP-decoder on the embeddings, which is very efficient. In contrast, \src receives the original source code as input and requires the fine-tuning of the transformer model, which takes more resources. The time complexity of \model depends on the number of aligned node-token pairs. Specifically, due to the node-token message passing mechanism, the time complexity of each node-token message passing step is linear to the number of aligned pairs, and such fine-grained interaction is performed for $L_2=6$ times as shown in Figure 1 of the main paper. The additional overhead incurred by these additional steps is shown to bring a performance gain in Section~\ref{sec-ablation}. All the methods in this paper can be trained on a single GPU, and we leave the scaling up of \model to leverage more expressive models as future work.


==> sec-result.tex <==
\section{More Results with Analysis}
\label{sec-more-results}

\subsection{Number of Solved Pairs Across Time}

\begin{figure}
\vspace*{-4mm}
     \centering
     \subfloat[\textbf{\human $Q_{32}$}]{\includegraphics[width=0.31\textwidth]{visualizations/human-32.png}}
     \subfloat[\textbf{\human $Q_{64}$}]{\includegraphics[width=0.31\textwidth]{visualizations/human-64.png}}
     \subfloat[\textbf{\human $Q_{128}$}]{\includegraphics[width=0.31\textwidth]{visualizations/human-128.png}}
\vspace*{-3mm}
     \centering
     \subfloat[\textbf{\hprd $Q_{32}$}]{\includegraphics[width=0.31\textwidth]{visualizations/hprd-32.png}}
     \subfloat[\textbf{\hprd $Q_{64}$}]{\includegraphics[width=0.31\textwidth]{visualizations/hprd-64.png}}
     \subfloat[\textbf{\hprd $Q_{128}$}]{\includegraphics[width=0.31\textwidth]{visualizations/hprd-128.png}}
\vspace*{-3mm}
%      \centering
%      \subfloat[\textbf{\dblp $Q_{32}$}]{\includegraphics[width=0.31\textwidth]{dblp-32.png}}
%      \subfloat[\textbf{\dblp $Q_{64}$}]{\includegraphics[width=0.31\textwidth]{dblp-64.png}}
%      \subfloat[\textbf{\dblp $Q_{128}$}]{\includegraphics[width=0.31\textwidth]{dblp-128.png}}
% \vspace*{-3mm}
     \centering
     \subfloat[\textbf{\eu $Q_{32}$}]{\includegraphics[width=0.31\textwidth]{visualizations/eu2005-32.png}}
     \subfloat[\textbf{\eu $Q_{64}$}]{\includegraphics[width=0.31\textwidth]{visualizations/eu2005-64.png}}
     \subfloat[\textbf{\eu $Q_{128}$}]{\includegraphics[width=0.31\textwidth]{visualizations/eu2005-128.png}}
\vspace*{-3mm}
     \centering
     \subfloat[\textbf{\youtube $Q_{32}$}]{\includegraphics[width=0.31\textwidth]{visualizations/youtube-32.png}}
     \subfloat[\textbf{\youtube $Q_{64}$}]{\includegraphics[width=0.31\textwidth]{visualizations/youtube-64.png}}
     \subfloat[\textbf{\youtube $Q_{128}$}]{\includegraphics[width=0.31\textwidth]{visualizations/youtube-128.png}}
     \caption{Comparison of the curves of the number of solved pairs versus time on \human, \hprd, \eu, and \youtube. The plot for \dblp are shown in the main text.}
     \label{fig:all-curves}
% \vspace*{-3mm}
\end{figure}

We provide figures on the number of solved pairs across time for all datasets in Figure~\ref{fig:all-curves}, showing that \sgmrlmodel consistently solves more query graph pairs than baseline methods on most datasets. Figure~\ref{fig:all-curves} also shows \sgmrlmodel's scalability with respect to query graph size, as baselines rapidly fail while \sgmrlmodel retains solid performance as query graphs get larger. Furthermore, the number of solutions found by baseline methods tend to flatten unlike \sgmrlmodel, which consistently solves more and more queries over time, suggesting that \sgmrlmodel will further outperform baselines if run for longer. We observe no clear correlation between the density of a query graph and the difficulty of solving the graph pair, i.e. the number of solutions found by the methods tested in our paper. We conjecture the difficulty is related to the distribution of the node degrees of a query graph, and leave the further investigation of predicting the difficulty of a graph pair without actually running a \task solver as future work.

\subsection{Results on Running Time}

We observe that the baseline solvers written in C++ have $O(1)$ time complexity for its random node selection policy for nodes in $G$, and thus tend to perform many more iterations than \sgmrlmodel written in Python during inference time.
% We report the total number of iterations and average running time per iteration for the methods tested in the main text. Since the baseline solvers are written in C++, and a fast random policy is adopted, they are much faster than \sgmrlmodel. 
However, even with many more iterations performed by these baselines, they still fail to solve most pairs due to the too large action space incurred by the 128-node query graphs. Although 128 nodes do not seem to be very large, due to the combinatorial nature of \task, the search space is still intractable for these fast baselines. In contrast, our model written in Python is slower for each iteration but offers a much better overall result, suggesting good practicality and the promising research direction of designing learning-based strategy to enhance search algorithms.

% \begin{table}[h]
% % \footnotesize
%   \begin{center}
%     \caption{Running time comparison on \dblp $Q_{128}$. The number of iterations is the averaged across the 100 pairs. ``ns'', ``ms'' denote nanoseconds and millisecond respectively. \yba{maybe just mention millions of iterations at high level}
%     }

    
%     \begin{tabular}{l|p{2.5cm}p{3cm}p{2cm}}
%     \label{table-timing}
%     \textbf{Model} & \textbf{\% Solved Pairs} & \textbf{\# Iterations} & \textbf{Time per Iter}\\
%     \hline
    
%     \qsi & 0.07 & 1092713998.89 & 274.55 ns \\ 
%     \gql & 0.02 & 459639.11 & 0.65 ms \\ 
%     \ceci & 0.18 & 1215745130.39 & 246.76 ns \\ 
%     \daf & 0.16 & 824427531.89 & 363.89 ns\\ 
%     \hybrid & 0.04 & 1928269226.84 & 155.58 ns \\ 
%     \nmatch & 0.04 & 24248.43 & 12.37 ms\\ 
    
%     \sgmrlmodel & \textbf{0.58} & 1724.06 & 174.01 ms\\ 
    
    
%     \end{tabular}
%   \end{center}
% % \vspace*{-4mm}
% \end{table}

We analyze the running time by showing the percentage of the major components in \sgmrlmodel. As shown in Figure~\ref{fig:pie}, without caching the intra-graph node embeddings, the propagation module is the bottleneck, due to its $\mathcal{O}(|E_q|+|E_G|)$ time complexity. It is noteworthy that we perform the propagation and matching modules sequentially to generate Figure~\ref{fig:pie} (a), i.e. for each \encoderlayer, we first run the propagation module and then run the matching module. Although it is possible to further optimize the implementation by running two modules in parallel (to be specific, the propagation module of layer $k$ and the matching module of layer $k-1$ could be performed in parallel on two devices), we argue the bottleneck would still be the propagation module, for which the proposed caching technique would help. In comparison, by caching the state-independent $\bm{h}_{\mathrm{intra}}^{(k)}$ node embeddings, the propagation module only takes $0.3\%$ (corresponding to the almost invisible slice of red color) of the total running time budget (5 minutes). 

\begin{figure}[h]
% \vspace*{-4mm}
     \centering
     \subfloat[\sgmrlmodel without caching of $\bm{h}_{\mathrm{intra}}^{(k)}$.]{\includegraphics[width=0.5\textwidth]{visualizations/pie_eu_no_caching.pdf}}
     \subfloat[\sgmrlmodel with caching of $\bm{h}_{\mathrm{intra}}^{(k)}$.]{\includegraphics[width=0.5\textwidth]{visualizations/pie_eu_caching.pdf}}
     \caption{Running time breakdown by executing \sgmrlmodel (the inference stage) on one randomly sampled graph pair from \eu for 5 minutes and collecting the running time spent on each component. With caching, more iterations are performed due to each iteration being much faster.}
     \label{fig:pie}
% \vspace*{-2mm}
\end{figure}


% \yba{also show CS and LCS changes across search iterations}
% \yba{mention average running time per iter?}

We plot the change of global candidate space (CS) size and the local candidate space (LCS) size across time in Figure~\ref{fig:cs-lcs}. Specifically, at each search iteration, a node $u_t$ from the query graph is chosen by $\phi$ (line 7 of Algorithm 1 in the main text), and the local candidate space is computed for $u_t$ (line 8 of Algorithm 1 in the main text). Therefore, we can record the number of candidates for $u_t$ in the global candidate space and in the local candidate space, and plot the change of CS and LCS sizes across search iterations. As shown in Figure~\ref{fig:cs-lcs}, there is a large reduction of candidate nodes from CS to LCS, suggesting the importance of computing a smaller local candidate space based on the current matching and the selected $u_t$. Without any LCS computation technique, the action space would be the global CS, which may contain up to $100,000$ nodes. Another important observation is that, the number of local candidate nodes varies dramatically across iterations. For example, in the initial iteration, since no nodes are matched, LCS is of the same size as CS, but as soon as one node pair is matched, the LCS computation can leverage the matched nodes by narrowing down the action space from all the nodes in CS to the first-order neighbors of the matched nodes. Existing LCS computation has several other techniques to reduce the candidate space size other than simply using the first-order neighbors of the matched subgraphs, and as a result, there can be less than 10 nodes in $\mathcal{A}_{u_t}$ in some iterations. However, when the search backtracks to an earlier state, there can be more candidate nodes in LCS, resulting in the varying LCS sizes across search.

\begin{figure}[h]
% \vspace*{-4mm}
     \centering
     \subfloat[\textbf{\human}]{\includegraphics[width=0.33\textwidth]{visualizations/human-cs.png}}
     \subfloat[\textbf{\hprd}]{\includegraphics[width=0.33\textwidth]{visualizations/hprd-cs.png}} \\
     \subfloat[\textbf{\dblp}]{\includegraphics[width=0.33\textwidth]{visualizations/dblp-cs.png}}
    \subfloat[\textbf{\eu}]{\includegraphics[width=0.33\textwidth]{visualizations/eu-cs.png}}
    \subfloat[\textbf{\youtube}]{\includegraphics[width=0.33\textwidth]{visualizations/youtube-cs.png}}
     \caption{Demonstration of the sizes of global candidate space (CS) and local candidate space (LCS) across search iterations, by running \sgmrlmodel on a randomly sampled graph pair from each dataset, and collecting the size of CS and LCS at each search iteration. The y-axis is in the log scale. We stop recording the CS and LCS sizes after 1000 search iterations.}%\yba{TODO: fix plots}}
     \label{fig:cs-lcs}
% \vspace*{-2mm}
\end{figure}

Since Figure~\ref{fig:cs-lcs} only shows the change of CS and LCS sizes across search for one graph pair, we show the statistics of CS and LCS sizes across 100 graph pairs in Table~\ref{table-cslcsstas}. Consistently with Figure~\ref{fig:cs-lcs}, the LCS size is on average smaller than the CS size, suggesting the importance of LCS computation.

\begin{table}[h]
% \footnotesize
  \begin{center}
    \caption{Statistics of the sizes of CS and LCS over 100 graph pairs for each dataset. ``Avg'', ``Min'', and ``Max'' denote average, minimum, and maximum, respectively.
    }
    
    \begin{tabular}{l|p{2cm}p{2cm}p{2cm}}
    \label{table-cslcsstas}
    \textbf{Dataset Name} & \textbf{Avg} & \textbf{Min} & \textbf{Max}\\
    \hline
    \textbf{\human $Q_{128}$ (CS)}  & 2217.65 & 395 & 4103 \\ 
    \textbf{\human $Q_{128}$ (LCS)}  & 55.65 & 0 & 1937 \\ \hline 
    \textbf{\hprd $Q_{128}$ (CS)}  & 4436.42 & 358 & 9031 \\ 
    \textbf{\hprd $Q_{128}$ (LCS)}  & 25.03 & 0 & 1911 \\ 
    \hline 
    \textbf{\dblp $Q_{128}$ (CS)}  & 170010.07 & 5370 & 317071 \\ 
    \textbf{\dblp $Q_{128}$ (LCS)}  & 23.34 & 0 & 62127 \\ 
    \hline 
    \textbf{\eu $Q_{128}$ (CS)}  & 612683.85 & 23327 & 861758 \\ 
    \textbf{\eu $Q_{128}$ (LCS)}  & 337.65 & 0 & 623730 \\ 
    \hline 
    \textbf{\youtube $Q_{128}$ (CS)}  & 368211.15 & 13248 & 1134773 \\
    \textbf{\youtube $Q_{128}$ (LCS)}  & 55.79 & 0 & 118752 \\
     
    \end{tabular}
  \end{center}
% \vspace*{-4mm}
\end{table}



% \yba{also mention batch operation for Q+U?}

\subsection{Results on Adapting \mcsrlmodel for \task}
\label{subsec=glsearchforsgm}

We report the performance of \sgmrlmodel and \mcsrlmodel on \task. As mentioned in Section~\ref{sec-related}, \task contains a tighter set of constraints than MCS, causing \mcsrlmodel's search framework to be less efficient and rely on a value-based model instead of a policy-based model. To measure the effects of both search framework and model design, we compare \sgmrlmodel to two models: (1) \mcsrlmodel, which uses the MCS search framework to conduct \task, and (2) \mcsrlmodeladapted, which uses the same value-based model architecture as \mcsrlmodel but adapted into \sgmrlmodel's search framework. To ensure the efficiency of value-based models, which need to execute an action before computing the $Q$ score, we adopt a simple sampling-based approach, where \mcsrlmodeladapted will always choose the best action out of up to 100 actions, regardless of the total action space size. We observe without such sampling, the model spends minutes executing a single action. Our results from Table~\ref{table-glsearch} emphasizes the differences between \task and MCS by confirming the criticality of \task search constraints and \sgmrlmodel's effective policy model design to \task performance.

\begin{table}[h]
% \footnotesize
\begin{center}
    \caption{Results of directly applying and adapting \mcsrlmodel originally designed for MCS detection to \task.}

    
    \begin{tabular}{l|lll}
    \label{table-glsearch}
    \textbf{Model} & \textbf{\dblp $Q_{32}$} & \textbf{\dblp $Q_{64}$} & \textbf{\dblp $Q_{128}$} \\
    \hline
    \sgmrlmodel & \textbf{1.00} & \textbf{0.97} & \textbf{0.58} \\ \hline
    \mcsrlmodel & 0.0 & 0.0 & 0.0 \\
    \mcsrlmodeladapted & 0.93 & 0.47 & 0.0 \\ 

    
    \end{tabular}
% \vspace*{-4mm}
\end{center}
\end{table}


\subsection{Reproducibility of Results}

We run the trained \sgmrlmodel model for 3 times to study the expected variance in model performance, due to the fixed running time budget used in experiments, and the fact that \sgmrlmodel tends to solve more pairs towards the end of the 5-minute budget for each pair as shown in Figure~\ref{fig:all-curves}. We find that \sgmrlmodel is able to reliably achieve good results on all datasets and outperform baseline methods. In contrast, baseline solvers in C++ tend to plateau and stop finding solutions for more pairs early in the 5-minute duration as seen in Figure~\ref{fig:all-curves}.

\begin{table}[h]
% \small
\footnotesize
  \begin{center}
    \caption{Reproducibility of the solved percentage results on the $Q_{128}$ datasets.
    }

    
    \begin{tabular}{l|ll}
    \label{table-acc}
    \textbf{Dataset} &\textbf{Mean} & \textbf{Stdev} \\
    \hline
    
    \textbf{\human $Q_{128}$} & 0.53 & 0.09 \\ 
    \textbf{\hprd $Q_{128}$} & 0.00 & 0.00 \\ 
    \textbf{\dblp $Q_{128}$} & 0.62 & 0.03 \\ 
    \textbf{\eu $Q_{128}$} & 0.23 & 0.03 \\
    \textbf{\youtube $Q_{128}$} & 0.11 & 0.01 \\ 
    
    % \textbf{\human $Q_{128}$} & 0.43 & 0.52* & 0.58* \\ 
    % \textbf{\hprd $Q_{128}$} & 0.00 & 0.00* & 0.00* \\ 
    % \textbf{\dblp $Q_{128}$} & 0.58 & 0.66 & 0.64 \\ 
    % \textbf{\eu $Q_{128}$} & 0.21 & 0.32* & 0.34* \\
    % \textbf{\youtube $Q_{128}$} & 0.11 & 0.10* & 0.14* \\ 
    
    % \hline
    
    % \textbf{\patents $Q_{32}$} & \textbf{0.78} & 0.16 & 0* & 0.67 & 0.19 & 0.20 & 0.52 \\ 
    % \textbf{\patents $Q_{64}$} & 0.54 & 0.27 & 0.00 & \textbf{0.64} & 0.00 & 0.31 & 0.61 \\ 
    % \textbf{\patents $Q_{128}$} & \textbf{0.24} & 0.00 & 0.00 & 0.00 & 0.00 & 0.00** & 0.03 \\ 

    \end{tabular}
  \end{center}
% \vspace*{-4mm}
\end{table}



\subsection{Results on Labeled Graphs for \task}

To test the generality of \sgmrlmodel, we compare it against baselines on a labeled dataset. By assigning labels, the filtering algorithm can further reduce the search space prior to the search process. Because of this, labeled datasets are generally easier than unlabeled datasets. The degree to which labels make \task easier is hard to determine. For instance, if all the target graph nodes in the same global candidate set share the same label, then the additional label constraint provides little guidance to search. On the other extreme, if each query graph node has a unique label that matches only one target graph node, then the search becomes trivial. For example, Knowledge Graph (KG) reasoning~\cite{ren2020query2box,zhang2021cone} can also be viewed as matching a subgraph in a large KG, where a first-order logical query is represented as directed acyclic graph. However, since the KG can be incomplete with missing relations, exact \task may not be the most appropriate choice~\cite{ren2020query2box}.

To be fair, we adopt the labeled \eu dataset provided by \cite{sun2020memory} for our experiment, where $|\Sigma|=10$. Note, we do not retrain \sgmrlmodel on the labeled dataset, opting to use the same model trained on the unlabelled dataset. While node labels are not reflected in the initial features of the graph, they do shrink the size of the global and local candidate set, as only nodes with the same label can match eachother.%\yba{how do we handle node labels in CS or LCS?}

\begin{table}[h]
\begin{center}
% \footnotesize
    \caption{Results on labeled \eu-labeled $Q_{32}$ dataset. The ratio of the number of solved pairs over the 100 pairs is reported.
    }

    
    \begin{tabular}{l|p{2cm}}%
    \label{table-labeled}
    \textbf{Model} & \textbf{\eu-labeled $Q_{32}$} \\
    \hline
    
    \qsi & 0.35 \\ 
    \gql & 0.72 \\ 
    \ceci & 0.70 \\ 
    \daf & 0.86 \\ 
    \hybrid & 0.82 \\ 
    % \nmatch & 0.08 \\ 
    \sgmrlmodel & \textbf{0.99} \\
    \end{tabular}
% \vspace*{-4mm}
\end{center}
\end{table}

As seen in Table\ref{table-labeled}, \sgmrlmodel outperforms baselines even on labeled graph instances, demonstrating its generality. This suggests the graph structure is very critical in \task search algorithms, even in the presence of other constraints such as node labels. We also tried such experiments on smaller datasets provided by \cite{sun2020memory}, but found all methods were able to solve the graph pairs. As seen in Table~\ref{table-cslcsstas}, adding node labels to graphs with already small candidate sets could drastically reduce the search space, such that search space pruning on its own is enough to find a valid solution; however, as we have demonstrated thus far, there are many non-trivial cases where a smarter search policy, such as \sgmrlmodel, is required for \task. It is also possible to further improve \sgmrlmodel performance by training it on the labeled dataset, but we leave this as future work.






% \subsection{Results on Finding All the Solutions for \task}
% \yba{mention limitation: can be faster}
% \yba{future directions: Parallelism? Even larger target graphs? Subgraph search in a database? Build an index?}

% \subsection{Results on Generalization of Trained Models}



% \subsection{Best Solution Sizes across Time}

% % \yba{TODO: running time on circuit (address running DVN too slow; time complexity; in practice can even use CPP with parallel to further speed up; overall training one day but can be applied to all testing pairs); KL}

% Figure~\ref{fig-iter-size} shows that under the budget we set, for the large real-world graph pairs, all the methods reach a ``steady state'' where the best solution found so far no longer grows. This means the search continues but the search cannot find a larger solution, illustrating the fact that search gets ``stuck''. In theory, given infinitely many iterations, all the models will eventually find the true MCS, which is the largest, but since the task is NP-hard, the search space can be exponential in the worst case (subject to pruning but in all the testing graph pairs the search has not finished yet), such budget has to be applied to search. 
% % This also illustrates the motivation for our backtracking using DQN outputs as detailed in Section~\ref{subsec-backtrack-dqn}.
% At the end of the 7500 iterations, though, all the models have made ``mistakes'' (visiting unpromising states) and in order to find even larger common subgraphs, the search needs to backtrack potentially many times to fix those ``mistakes'' (backtracking to a very early state). 
% % Since all methods will eventually find the same true MCS given infinitely many iterations, 

% Admittedly, there is always the possibility that for more iterations, some baseline method may find a larger solution. Besides, in each iteration \mcsrlmodel does take more running time overhead as shown in Table~\ref{table-additional-runtime}. However, the point of our model is to quickly find a larger solution in as few iterations as possible, not to find a large solution given too many iterations. In other words, the goal of \mcsrlmodel is to be \textbf{smart} enough to \textbf{quickly} find a large solution instead of purely finding a good solution. Figure~\ref{fig-iter-size} shows that \mcsrlmodel not only finds solutions larger than baselines \textit{when} the 7500 iterations budget is reached but also finds larger solutions faster than baselines \textit{before} the budget is reached.


% \begin{table}[h]
% \small
%   \begin{center}
%     \caption{Average running time per iteration (msec).}
%     \begin{tabular}{l|llllllll}
%     \label{table-additional-runtime}
%     \textbf{Method}&
%     \textbf{\road} &
%     \textbf{\kgen} &
%     \textbf{\kgzh} &
%     \textbf{\kgenzh} &
%     \textbf{\enron} &
%     \textbf{\amazon} &
%     \textbf{\circuit} &
%     \textbf{\ppi} \\
%     \hline
%     \mcsp         & 2.040  & 10.724 & 1.415  & 0.974  & 1.722   & 2.891  & 1.776   & 0.498 \\
%     \mcsprl      & 0.894  & 6.834  & 2.103  & 1.247  & 2.166   & 3.107  & 2.080   & 0.559  \\
%     \hline
%     \gwqap        & 0.548  & 0.834  & 0.546  & 4.692  & 1.041   & 3.419  & 1.550   & 0.546 \\
%     \pca          & 1.152  & 1.797  & 0.967  & 0.897  & 1.739   & 2.725  & 3.792   & 0.636  \\
%     \mcstreemodel & 2.394  & 4.172  & 4.648  & 5.667  & 9.610   & 9.788  & 7.471   & 15.742 \\
%     \hline
%     \randq        & 17.392 & 66.418 & 67.342 & 67.946 & 163.005 & 71.972 & 655.447 & 83.488 \\
%     \mcsrlmodel   & 8.132  & 66.552 & 71.409 & 96.262 & 135.087 & 51.181 & 37.377  & 60.509 \\
%     % \hline
%     \end{tabular}
%   \end{center}
% \vspace*{-4mm}
% \end{table}

% % \begin{table*}[h]
% % % \small
% %   \begin{center}
% %     \caption{TODO}
% %     \begin{tabular}{l|cccccccc}
% %     \label{table-acc}
% %     \textbf{Method} &
% %     \textbf{\road} &
% %     \textbf{\kgen} &
% %     \textbf{\kgzh} &
% %     \textbf{\kgenzh} &
% %     %\textbf{\facebook} &
% %     \textbf{\enron} &
% %     \textbf{\amazon} &
% %     \textbf{\circuit} &
% %     \textbf{\ppi} \\
% %       \hline
% %       \mcsrlmodel $(N_b = 1; N_d = 10)$ & 115 & 508 & \textbf{513} & \textbf{527} & 519 & \textbf{842} & 3419 & 399 \\
% %       \mcsrlmodel $(N_b = 1; N_d = 20)$ & 131 & 508 & 482 & 521 & \textbf{543} & 791 & 3515 & \textbf{404} \\
% %       \mcsrlmodel $(N_b = 1; N_d = 30)$ & \textbf{149} & \textbf{510} & 484 & 520 & 507 & 784 & \textbf{4219} & 397 \\
% %       \hline
% %       \mcsrlmodel $(N_b = 1; N_d = 10)$ & 115 & 508 & \textbf{513} & \textbf{527} & 519 & \textbf{842} & \textbf{3419} & \textbf{399} \\
% %       \mcsrlmodel $(N_b = 2; N_d = 20)$ & 122 & 494 & 464 & 517 & 540 & 819 & 2206 & 395 \\
% %       \mcsrlmodel $(N_b = 3; N_d = 30)$ & \textbf{155} & \textbf{515} & 500 & 500 & \textbf{1422} & 796 & 2189 & 386 \\
% %     \end{tabular}
% %   \end{center}
% % \vspace*{-6mm}
% % \end{table*}


% \begin{figure}
%      \centering
%      \subfloat[\road]{\includegraphics[width=0.5\textwidth]{vis/Road.png}}
%      \subfloat[\kgen]{\includegraphics[width=0.5\textwidth]{vis/DbEn.png}}
%      \newline
%      \vspace*{-4mm}

%      \subfloat[\kgzh]{\includegraphics[width=0.5\textwidth]{vis/DbZh.png}}
%      \subfloat[\kgenzh]{\includegraphics[width=0.5\textwidth]{vis/Dbpd.png}}
%      \newline
%      \vspace*{-4mm}

%      \subfloat[\enron]{\includegraphics[width=0.5\textwidth]{vis/Enro.png}}
%      \subfloat[\amazon]{\includegraphics[width=0.5\textwidth]{vis/CoPr.png}}
%      \newline
%      \vspace*{-4mm}

%      \subfloat[\circuit]{\includegraphics[width=0.5\textwidth]{vis/Circ.png}}
%      \subfloat[\ppi]{\includegraphics[width=0.5\textwidth]{vis/HPpi.png}}
%      \caption{For each method, we maintain the best solution found so far in each iteration during the search process. We plot the size of the largest extracted common subgraphs found so far vs search iteration count for all the methods across all the datasets. The larger the subgraph size, the better (``smarter'') the model in terms of quickly finding a large MCS solution under limited budget for large graphs.}
%      \label{fig-iter-size}
% \end{figure}


% % \begin{figure}
% % % \vspace{-1.8em}
% %     \centering
% %     \subfloat[On AIDS. Different colors represent different node labels.]
% %     {{\includegraphics[scale=0.37]{vis/Road.png} }}
% %     \vspace{-0.0in}
% %     \centering
% %     \subfloat[On LINUX.]
% %     {{\includegraphics[scale=0.37]{vis/DbEn.png} }}
% %     \vspace{-0.0in}
% %     \centering
% %     \subfloat[On IMDB.]
% %     {{\includegraphics[scale=0.37]{vis/DbZh.png} }}
% %     \vspace{-0.0in}
% %     \caption{Query case studies.}
% %     \label{fig-iter-size}
% % % \vspace{-2.8em}    
% % \end{figure}


% In addition to reaching a larger solution is less iterations, \mcsrlmodel also reaches better solutions with respect to runtime, as shown in Figure~\ref{fig-time-size}. Notice, \mcsrlmodel finds the same large subgraph in 10 minutes as in 7500 iterations. Although per iteration, it is slower than \mcsp per iteration, \mcsrlmodel finds a larger solution in usually less than a minute. Moreover, our implementation can be further optimized. Note, we adapted all baselines to run on Python for fair comparison, and made sure the search iteration counting is consistent across all baselines and the results shown in the main text. At this stage, our main goal is to explore the idea of \textit{\textbf{``learning to search''}}, which has been experimentally verified to be a promising direction of research, and leave the efforts of implementation optimization using various techniques as future focus.

% % Although our goal is to design a model to reach larger solutions in less iterations, and our real running time is slower compared to simpler heuristics-based algorithms, we still compare the subgraph growth vs running time of \mcsp and \mcsrlmodel in Figure~\ref{fig-time-size} under a budget of 10 minutes. Notice, \mcsrlmodel finds the same large subgraph in 10 minutes as in 7500 iterations. Although per iteration, it is slower than \mcsp per iteration, \mcsrlmodel finds a larger solution in usually less than a minute. Moreover, our implementation can be further optimized which can be left as future work. Note that for \mcsprl, it is implemented in C++, and we have currently only adapted \mcsp into our Python framework for a fair real time evaluation. We do make sure the search iteration counting is consistent across the C++ and Python implementations, which is the results shown in the main text. At this stage, our main goal is to explore the idea of \textit{\textbf{``learning to search''}}, which has been experimentally verified to be a promising direction of research, and leave the efforts of implementation optimization using various techniques as future focus.




% \begin{figure}
%      \centering
%      \subfloat[\road]{\includegraphics[width=0.5\textwidth]{vis/Road_time.png}}
%      \subfloat[\kgen]{\includegraphics[width=0.5\textwidth]{vis/DbEn_time.png}}
%      \newline
%      \vspace*{-4mm}

%      \subfloat[\kgzh]{\includegraphics[width=0.5\textwidth]{vis/DbZh_time.png}}
%      \subfloat[\kgenzh]{\includegraphics[width=0.5\textwidth]{vis/Dbpd_time.png}}
%      \newline
%      \vspace*{-4mm}

%      \subfloat[\enron]{\includegraphics[width=0.5\textwidth]{vis/Enro_time.png}}
%      \subfloat[\amazon]{\includegraphics[width=0.5\textwidth]{vis/CoPr_time.png}}
%      \newline
%      \vspace*{-4mm}

%      \subfloat[\circuit]{\includegraphics[width=0.5\textwidth]{vis/Circ_time.png}}
%      \subfloat[\ppi]{\includegraphics[width=0.5\textwidth]{vis/HPpi_time.png}}
%      \caption{For each method, we maintain the best solution found so far in each iteration during the search process. We plot the size of the largest extracted common subgraphs found so far vs the real running time for all the methods across all the datasets. The larger the subgraph size, the better (``smarter'') the model in terms of quickly finding a large MCS solution under limited budget for large graphs.}
%      \label{fig-time-size}
% \end{figure}




% \subsection{Additional Ablation Study}

% Table~\ref{table-abl-ptil} shows that pre-training and imitation learning benefit the performance under four out of the eight datasets. On \enron and \ppi, without pre-training, our model performs better, which may be attributed to the fact that they are dense graphs (Table~\ref{table-test-data}) while the training graphs used in stage 1 are relatively small and sparse (Section~\ref{subsec-cur-learning}).

% \begin{table}[h]
% \small
%   \begin{center}
%     \caption{Contribution of pre-training and imitation learning to the performance of \mcsrlmodel. ``no-sup'' denotes the removal of the pre-training stage (The first 3750 iterations: IL; The last 6250 iterations: Normal QDN training); ``no IL'' denotes the removal of the imitation learning stage (The first 3750 iterations: pre-training; The last 6250 iterations: normal DQN training); ``no sup; no IL'' indicates the entire training (10000 iterations) is normal DQN training.}
    
%     \begin{tabular}{l|llllllll}
%     \label{table-abl-ptil}
%     % \multirow{}{} 
%     \textbf{Method}&
%     \textbf{\road} &
%     \textbf{\kgen} &
%     \textbf{\kgzh} &
%     \textbf{\kgenzh} &
%     %\textbf{\facebook} &
%     \textbf{\enron} &
%     \textbf{\amazon} &
%     \textbf{\circuit} &
%     \textbf{\ppi} \\
%     \hline
% \mcsrlmodel (no sup) & 0.557 & 0.957 & 0.946 & 0.904 & \textbf{1.000} & 0.999 & \textbf{1.000} & \textbf{1.000} \\
% \mcsrlmodel (no IL) & \textbf{1.000} & 0.933 & 0.965 & 0.887 & 0.357 & 0.875 & 0.666 & 0.632 \\
% \mcsrlmodel (no sup; no IL) & 0.678 & 0.907 & 0.896 & 0.837 & 0.401 & 0.949 & 0.949 & 0.651 \\
%     \hline
%     \mcsrlmodel & 0.879 & \textbf{1.000} & \textbf{1.000} & \textbf{1.000} & 0.412 &\textbf{1.000} & 0.855 & 0.688\\
%     \hline
%     \hline
%     \nnodes & 149 & 486 & 465 & 471 & 1318 & 790 & 4112 & 587 \\
%     \end{tabular}
%   \end{center}
% \vspace*{-4mm}
% \end{table}





% Table~\ref{table-abl-promise} shows that the promised-based search improves the performance under four out of the eight datasets. For the other four datasets, the performance does not change, indicating that the backtracking to an earlier promising state based on the DQN output at least does not hurt the performance. In the cases like \enron and \ppi, whose average node degrees are large, the promise-based search improves the performance by a large amount, showing the usefulness of the proposed strategy.

% \begin{table}[h]
% \small
%   \begin{center}
%     \caption{Contribution of promise-based search (Section~\ref{subsec-backtrack-dqn}) to the performance of \mcsrlmodel. ``no promise'' denotes that the search does not use the proposed promise-based search, i.e. it does not backtrack to an earlier state if the search makes no progress after a certain amount of iterations, and instead, it continues the regular branch and bound search.}
    
%     \begin{tabular}{l|llllllll}
%     \label{table-abl-promise}
%     % \multirow{}{} 
%     \textbf{Method}&
%     \textbf{\road} &
%     \textbf{\kgen} &
%     \textbf{\kgzh} &
%     \textbf{\kgenzh} &
%     %\textbf{\facebook} &
%     \textbf{\enron} &
%     \textbf{\amazon} &
%     \textbf{\circuit} &
%     \textbf{\ppi} \\
%     \hline
%     \mcsrlmodel (no promise) & 0.879 & \textbf{1.000} & \textbf{1.000} & \textbf{1.000} & 0.412 &\textbf{1.000} & 0.855 & 0.688 \\
%     \hline
%     \mcsrlmodel & \textbf{1.000} & \textbf{1.000} & \textbf{1.000} & \textbf{1.000} & \textbf{1.000} &\textbf{1.000} & \textbf{1.000} & \textbf{1.000} \\
%     \hline
%     \hline
%     \nnodes & 131 & 508 & 482 & 521 & 543 & 791 & 3515 & 404 \\
%     \end{tabular}
%   \end{center}
% \vspace*{-4mm}
% \end{table}


% \subsection{Scalability Study}

% \mcsrlmodel can scale to very large graphs containing tens of thousands of nodes. To verify this, we generate 6 large synthetic graphs (3 graph pairs) using the BA, ER, and WS algorithms, each with 10000 nodes, and ran \mcsrlmodel against heuristic-based baselines for 7500 iterations. Our model is superior in all instances, as shown in Table~\ref{table-scal-study}.

% \begin{table}[h]
% \small
%   \begin{center}
%     \caption{Results of \mcsrlmodel to even larger networks. Each synthetic dataset consists of one graph pair labeled as $\langle$generation algorithm$\rangle$-$\langle$number of nodes in each graph$\rangle$. For BA graphs, we set the edge density to 4. For ER graphs, we set the edge density to 0.0016. For WS graphs, we set the rewiring probability to 0.2 and ring density to 4.}
    
%     \begin{tabular}{l|lll}
%     \label{table-scal-study}
%     % \multirow{}{} 
%     \textbf{Method}&
%     \textbf{BA-10k} &
%     \textbf{ER-10k} &
%     \textbf{WS-10k} \\
%     \hline
% \mcsp & 0.952 & 0.975 & 0.911 \\
% \mcsprl & 0.964 & 0.975 & 0.911 \\
%     \hline
%     \mcsrlmodel & \textbf{1.000} & \textbf{1.000} & \textbf{1.000} \\
%     \hline
%     \hline
%     \nnodes & 3172 & 2190 & 4839 \\
%     \end{tabular}
%   \end{center}
% \vspace*{-4mm}
% \end{table}


% % \mcsrlmodel will retain consistent performance as graph size increases, but heuristic baselines will start to fail, as a smarter policy is required as graph sizes scale up. We validate this claim through constructing 6 new datasets from the circuit dataset, \circuit, sampling isomorphic subgraphs with differing numbers of nodes. In this case, we know the ground truth MCS, which is the whole graph. We ran \mcsrlmodel against heuristic-based baselines for 7500 iterations, and find \mcsrlmodel outperforms heuristic baselines in all experiments, significant performance advantage (~2x performance) begins once graphs are larger than 256 nodes, and our model consistently matches almost the entire graph

% % \begin{table}[h]
% % \small
% %   \begin{center}
% %     \caption{TODO}
    
% %     \begin{tabular}{l|lllllll}
% %     \label{table-abl-ptil}
% %     % \multirow{}{} 
% %     \textbf{Method}&
% %     \textbf{\circuit -128} &
% %     \textbf{\circuit -256} &
% %     \textbf{\circuit -512} &
% %     \textbf{\circuit -1024} &
% %     \textbf{\circuit -2048} &
% %     \textbf{\circuit -4096} &
% %     \textbf{\circuit (4275)} \\
% %     \hline
% % \mcsp & 0.812  & 0.559  & 0.281 & 0.282 & 0.480 & 0.645 & 0.498 \\
% % \mcsprl & 0.812  & 0.559  & 0.269 & 0.432 & 0.476 & 0.633 & 0.583 \\
% %     \hline
% %     \mcsrlmodel & \textbf{1.000} & \textbf{1.000} & \textbf{1.000}  & \textbf{1.000} & \textbf{1.000} & \textbf{1.000} & \textbf{1.000} \\
% %     \hline
% %     \hline
% %     \nnodes & 128 & 256 & 509 & 999 & 2040 & 4033 & 3515 \\
% %     \end{tabular}
% %   \end{center}
% % \vspace*{-4mm}
% % \end{table}

% \subsection{Results on Graph Pairs with Known MCS Size Lower Bound}


% To better understand the quality of subgraphs found by \mcsrlmodel, we construct new datasets with known lower bound MCS sizes. This is accomplished through generating 2 new graphs that share a common subgraph from the existing large real-world graph datasets. For each real-world graph, $\mathcal{G}_0$, we randomly extract 3 different subgraphs of the same size, $\mathcal{S}_0$, $\mathcal{S}_1$, and $\mathcal{S}_2$, by running breadth first search from 3 different starting nodes and extracting the explored induced subgraph. To construct a new graph pair, ($\mathcal{G}_1$, $\mathcal{G}_2$), we form $\mathcal{G}_1$ by connecting $\mathcal{S}_0$ to $\mathcal{S}_1$ with 20 random edges and form $\mathcal{G}_2$ by connecting $\mathcal{S}_0$ to $\mathcal{S}_2$ with 20 random edges. Thus, connections between $\mathcal{S}_0$ nodes are the same in both $\mathcal{G}_1$ and $\mathcal{G}_2$, but connections between $\mathcal{G}_1 \setminus \mathcal{S}_0$ and $\mathcal{G}_2 \setminus \mathcal{S}_0$ are different. Notice, the lower bound of MCS size in these new datasets would be $|\mathcal{S}_0|$, and we name the new dataset by adding `ss' to the parent dataset's name.


% \begin{table}[h]
% \small
%   \begin{center}
%     \caption{Results on graph pairs with a common core subgraph (lower bound of MCS), with a fixed runtime of 10 minutes.}

    
%     \begin{tabular}{l|llllll}
%     \label{table-acc}
%     \multirow{2}{*}{\textbf{Method}} &
%     \textbf{\road-ss} &
%     \textbf{\kgen-ss} &
%     \textbf{\kgzh-ss} &
%     \textbf{\enron-ss} &
%     \textbf{\amazon-ss} &
%     \textbf{\ppi-ss} \\
%     & 444 & 778 & 762 & 1346 & 1406 & 860 \\
%          \hline
%     \mcsp         & 0.588   & 0.466   & 0.544   & 0.216   & 1.000   & 0.233  
% \\
%     \mcsprl       & 0.588   & 0.466   & 0.544   & 0.214   & 1.000   & 0.233 \\
%     \hline
%     \mcsrlmodel   & \textbf{1.000} & \textbf{1.000} & \textbf{1.000} & \textbf{1.000} & \textbf{1.000} & \textbf{1.000} \\
%     \hline
%     \hline
%     \nnodes & 187     & 388     & 349     & 672     & 702     & 429    \\
%     \textsc{Core (Lower Bound) Size} & 222     & 389     & 381     & 673     & 703     & 430    \\
%     \end{tabular}
%   \end{center}
% \vspace*{-4mm}
% \end{table}


==> sec-vis.tex <==

\section{Dataset Visualizations}
\label{sec-vis}




%\subsection{Dataset}

As mentioned in the main paper, there are 35 kernels (programs) in \vTwoFalse and 26 kernels (programs) in \vTwoTrue. Specifically, \vTwoFalse consists of the following kernels (programs): \textsc{2mm, aes, atax, bicg, bicg-large, covariance, doitgen, doitgen-r, fdtd-2d-l, gemm-blocked, gemm-n, gemm-p, gemm-p-l, gemver, gesummv, mvt, nw, spmv-crs, spmv-ellpack, stencil, stencil-3d, symm, symm-opt, syrk, trmm}, and \textsc{trmm-opt}; \vTwoTrue consists of the following kernels (programs): \textsc{2mm, 3mm, adi, aes, atax, atax-medium, bicg, bicg-medium, correlation, doitgen, doitgen-r, fdtd-2d, gemm-blocked, gemm-n, gemm-p, gemver, gesummv, gesummv-medium, heat-3d, jacobi-1d, jacobi-2d, md, mvt, mvt-medium, nw, seidel-2d, spmv-crs, spmv-ellpack, stencil, stencil-3d, symm, syr2k, syrk, trmm}, and \textsc{trmm-opt}.

The source code for \twomm is shown in Code~\ref{code:2mm} with its CDFG shown in Figure~\ref{fig-vis-2mm}.



%\begin{wrapfigure}{r}
\small
% \begin{wrapfigure}{r}{0.5\textwidth}
% \begin{minipage}[t]{0.5\textwidth}
% \vspace{-0.12in}
\begin{lstlisting}[language=C,caption={\small{Code snippet of the \twomm kernel (program).
}},label={code:2mm},floatplacement=H]
#pragma ACCEL kernel

void kernel_2mm(int ni,int nj,int nk,int nl,double alpha,double beta,double tmp[40][50],double A[40][70],double B[70][50],double C[50][80],double D[40][80])
{
  int i;
  int j;
  int k;
//#pragma scop
/* D := alpha*A*B*C + beta*D */
  
#pragma ACCEL PIPELINE auto{__PIPE__L0}
  
#pragma ACCEL TILE FACTOR=auto{__TILE__L0}
  
#pragma ACCEL PARALLEL FACTOR=auto{__PARA__L0}
  for (i = 0; i < 40; i++) {
    
#pragma ACCEL PIPELINE auto{__PIPE__L2}
    
#pragma ACCEL TILE FACTOR=auto{__TILE__L2}
    
#pragma ACCEL PARALLEL FACTOR=auto{__PARA__L2}
    for (j = 0; j < 50; j++) {
      tmp[i][j] = 0.0;
      
#pragma ACCEL PARALLEL reduction = tmp FACTOR=auto{__PARA__L4}
       for (k = 0; k < 70; ++k) {
       tmp[i][j] += alpha * A[i][k] * B[k][j];
      }
    }
  }
  
#pragma ACCEL PIPELINE auto{__PIPE__L1}
  
#pragma ACCEL TILE FACTOR=auto{__TILE__L1}
  
#pragma ACCEL PARALLEL FACTOR=auto{__PARA__L1}
  for (i = 0; i < 40; i++) {
    
#pragma ACCEL PIPELINE auto{__PIPE__L3}
    
#pragma ACCEL TILE FACTOR=auto{__TILE__L3}
    
#pragma ACCEL PARALLEL FACTOR=auto{__PARA__L3}
    for (j = 0; j < 80; j++) {
      D[i][j] *= beta;
      
#pragma ACCEL PARALLEL reduction = D FACTOR=auto{__PARA__L5}
      for (k = 0; k < 50; ++k) {
        D[i][j] += tmp[i][k] * C[k][j];
      }
    }
  }
//#pragma endscop
}
\end{lstlisting}
% \vspace{-0.15in}
% \end{minipage}
% \end{wrapfigure}
\normalsize







The source code for \cov is shown in Code~\ref{code:cov} with its CDFG shown in Figure~\ref{fig-vis-cov}.



%\begin{wrapfigure}{r}
\small
% \begin{wrapfigure}{r}{0.5\textwidth}
% \begin{minipage}[t]{0.5\textwidth}
% \vspace{-0.12in}
\begin{lstlisting}[language=C,caption={\small{Code snippet of the \cov kernel (program).
}},label={code:cov},floatplacement=H]
#pragma ACCEL kernel

void kernel_covariance(int m,int n,double float_n,double data[100][80],double cov[80][80],double mean[80])
{
  int i;
  int j;
  int k;
//#pragma scop
  
#pragma ACCEL PIPELINE auto{__PIPE__L0}
  
#pragma ACCEL TILE FACTOR=auto{__TILE__L0}
  
#pragma ACCEL PARALLEL FACTOR=auto{__PARA__L0}
  for (j = 0; j < 80; j++) {
    mean[j] = 0.0;
    
#pragma ACCEL PARALLEL reduction=mean FACTOR=auto{__PARA__L3}
    for (i = 0; i < 100; i++) {
      mean[j] += data[i][j];
    }
    mean[j] /= float_n;
  }
  
#pragma ACCEL PIPELINE auto{__PIPE__L1}
  
#pragma ACCEL TILE FACTOR=auto{__TILE__L1}
  
#pragma ACCEL PARALLEL FACTOR=auto{__PARA__L1}
  for (i = 0; i < 100; i++) {
    
#pragma ACCEL PARALLEL reduction=data FACTOR=auto{__PARA__L4}
    for (j = 0; j < 80; j++) {
      data[i][j] -= mean[j];
    }
  }
  
#pragma ACCEL PIPELINE auto{__PIPE__L2}
  
#pragma ACCEL TILE FACTOR=auto{__TILE__L2}
  
#pragma ACCEL PARALLEL FACTOR=auto{__PARA__L2}
  for (i = 0; i < 80; i++) {
    
#pragma ACCEL PIPELINE auto{__PIPE__L5}
    for (j = i; j < 80; j++) {
      cov[i][j] = 0.0;
      
#pragma ACCEL PARALLEL reduction=cov FACTOR=auto{__PARA__L6}
      for (k = 0; k < 100; k++) {
        cov[i][j] += data[k][i] * data[k][j];
      }
      cov[i][j] /= float_n - 1.0;
      cov[j][i] = cov[i][j];
    }
  }
//#pragma endscop
}
\end{lstlisting}
% \vspace{-0.15in}
% \end{minipage}
% \end{wrapfigure}
\normalsize





The source code for \trmmOpt is shown in Code~\ref{code:trmm-opt} with its CDFG shown in Figure~\ref{fig-vis-trmm-opt}.



%\begin{wrapfigure}{r}
\small
% \begin{wrapfigure}{r}{0.5\textwidth}
% \begin{minipage}[t]{0.5\textwidth}
% \vspace{-0.12in}
\begin{lstlisting}[language=C,caption={\small{Code snippet of the \trmmOpt kernel (program).
}},label={code:trmm-opt},floatplacement=H]
#pragma ACCEL kernel

void kernel_trmm(double alpha,double A[60][60],double B[60][80])
{
//BLAS parameters
//SIDE   = 'L'
//UPLO   = 'L'
//TRANSA = 'T'
//DIAG   = 'U'
// => Form  B := alpha*A**T*B.
// A is MxM
// B is MxN
  
#pragma ACCEL PIPELINE auto{__PIPE__L0}
  
#pragma ACCEL TILE FACTOR=auto{__TILE__L0}
  
#pragma ACCEL PARALLEL FACTOR=auto{__PARA__L0}
  for (int i = 0; i < 60; i++) {
    
#pragma ACCEL PIPELINE auto{__PIPE__L1}
    
#pragma ACCEL TILE FACTOR=auto{__TILE__L1}
    
#pragma ACCEL PARALLEL FACTOR=auto{__PARA__L1}
    for (int j = 0; j < 80; j++) {
      double sum = B[i][j];
#pragma ACCEL PARALLEL reduction=sum FACTOR=auto{__PARA__L2}
      for (int k = 0; k < 60; k++) {
        if (k > i) {
          sum += A[k][i] * B[k][j];
        }
      }
      B[i][j] = alpha * sum;
    }
  }
}
\end{lstlisting}
% \vspace{-0.15in}
% \end{minipage}
% \end{wrapfigure}
\normalsize



\begin{figure}[h]
\centering
    \includegraphics[width=0.6\textwidth]{vis/vis-2mm-cdfg.png}
    \caption{Visualization of the CDFG for the \twomm program. Node colors indicate the block attribute derived from the assembly code. Edge colors indicate the flow attribute.}
    \label{fig-vis-2mm}
\end{figure}

\begin{figure}[h]
\centering

    \includegraphics[width=0.6\textwidth]{vis/cov-cdfg.png}
    \caption{Visualization of the CDFG for the \cov program. Node colors indicate the block attribute derived from the assembly code. Edge colors indicate the flow attribute.}
    \label{fig-vis-cov}
\end{figure}


\begin{figure}[h]
\centering
    \includegraphics[width=0.6\textwidth]{vis/trmm-opt-cdfg.png}
    \caption{Visualization of the CDFG for the \trmmOpt program. Node colors indicate the block attribute derived from the assembly code. Edge colors indicate the flow attribute.}
    \label{fig-vis-trmm-opt}
\end{figure}




